Photorealistic Facial Texture Inference Using Deep Neural Networks

We present a data-driven inference method that can synthesize a photorealistic texture map of a complete 3D face model given a partial 2D view of a person in the wild. After an initial estimation of shape and low-frequency albedo, we compute a high-frequency partial texture map, without the shading component, of the visible face area. To extract the fine appearance details from this incomplete input, we introduce a multi-scale detail analysis technique based on mid-layer feature correlations extracted from a deep convolutional neural network. We demonstrate that fitting a convex combination of feature correlations from a high-resolution face database can yield a semantically plausible facial detail description of the entire face. A complete and photorealistic texture map can then be synthesized by iteratively optimizing for the reconstructed feature correlations. Using these high-resolution textures and a commercial rendering framework, we can produce high-fidelity 3D renderings that are visually comparable to those obtained with state-of-the-art multi-view face capture systems. We demonstrate successful face reconstructions from a wide range of low resolution input images, including those of historical figures. In addition to extensive evaluations, we validate the realism of our results using a crowdsourced user study.

==> tables/lightstage_pca_ours.tex <==
\begin{table}[]
\centering
\caption{Order of quality given by 100 testers on 3 different subjects (307 records in total).}
\label{tbl:user_study_lightstage}
\begin{tabular}{rc}
\hline
\multicolumn{1}{c}{order}                     & count \\ \hline
Ours $>$ LightStage $>$ PCA & 124   \\
LightStage $>$ Ours $>$ PCA & 81    \\
Ours $>$ PCA $>$ LightStage & 15    \\
LightStage $>$ PCA $>$ Ours & 22    \\
PCA $>$ Ours $>$ LightStage & 33    \\
PCA $>$ LightStage $>$ Ours & 32    \\ \hline
\end{tabular}
\end{table}
